Investigating the Effectiveness of HyperTuning via Gisting

Gisting (Mu et al., 2023) is a simple method for training models to compress information into fewer token representations using a modified attention mask, and can serve as an economical approach to training Transformer-based hypernetworks. We introduce HyperLlama, a set of Gisting-based hypernetworks built on Llama-2 models that generates task-specific soft prefixes based on few-shot inputs. In experiments across P3, Super-NaturalInstructions and Symbol Tuning datasets, we show that HyperLlama models can effectively compress information from few-shot examples into soft prefixes. However, they still underperform multi-task fine-tuned language models with full attention over few-shot in-context examples. We also show that HyperLlama-generated soft prefixes can serve as better initializations for further prefix tuning. Overall, Gisting-based hypernetworks are economical and easy to implement, but have mixed empirical performance.

==> discarded/conclusion.tex <==
\section{Thesis Conclusion}

In this dissertation, we have outlined a set of work studying approaches to imparting knowledge and skills to increasingly capable language models.
Pretrained language models have been shown to be tremendous foundations for building 

such as language understanding, machine translation, and chat applications.
After pretraining, models often undergo one or several additional stages of training to adapt them to a specific application or reduce undesirable behaviors, often referred to as "post-training" by practitioners. Methods involved in post-training include task-specific fine-tuning \cite{ulmfit,gpt1}, instruction tuning \cite{t0,flan}, and RLHF \cite{rlhf}.

This dissertation includes a body of work studying how knowledge is imparted into models during this second stage of training.
In Chapter 2, we began by examining a simple method for transfer learning: intermediate training, or sequentially fine-tuning on an intermediate and then the target task. 
In experiments on BERT \cite{bert} found the intermediate training with the right tasks leads to improved downstream performance as well as more stable training, particularly for downstream tasks with limited training data.
Certain tasks like MNLI \cite{MNLI} are found to have positive transfer to a large number of downstream tasks.
Intermediate training thus serves as a simple but effective approach for improving downstream performance.

However, there are cases where intermediate training can negatively impact downstream task performance.
Being able to identify intermediate tasks that transfer positively to downstream task is thus of great importance.
In Chapter 3, we followed up by exploring when and why intermediate task transfer is successful, by identifying what factors determine whether an intermediate task will be beneficial for a given downstream task.
To assist in this investigation, we introduce a third set of tasks: probing tasks, which are intentionally constructed tasks that capture a specific linguistic property or skill.
\todo{By using the probing tasks as a additional correlate, we} 
While we fail to cleanly identify 

Beyond performance on English tasks, language models pretrained on data in a large number of languages have also been shown to perform well on tasks across different languages.
One interesting property of such multilingual models is zero-shot cross-lingual transfer, wherein a model fine-tuned on data from a given task in language A can perform well on data from the same task in another language B, despite never being trained on task data in language B.
In Chapter 4, we apply intermediate training to the zero-shot cross-lingual transfer setting as well, applying two stages of fine-tuning on tasks in English before evaluating the models on unseen task-language pairs.
We find that intermediate training similarly leads to improvements in zero-shot cross-lingual transfer with the XLM-R models on the XTREME benchmark.
This demonstrates the wide applicability of intermediate training to transfering knowledge across tasks.

In the latter section of this dissertation, we turned our attention toward hypernetworks \cite{}, focusing on using specially trained language models (the \textit{hypernetwork}) to generate parameters that can be embedded in a downstream frozen language model.
In doing so, we can transfer knowledge captured by the hypernetwork and compress it into a small number of parameters, taking advantage of the modular nature of neural networks.
In Chapter 5, we introduced \citet{HyperTuning}, a method for using an LLM-based hypernetwork to generate task-specific parameters based on a small set of in-context few-shot examples.
The advantage of this approach is two-fold: generate parameters using only a forward pass, and efficiency advantages from compressing task-relevant information from task examples into a fixed-sized set of parameters.
We demonstrated this approach by training HyperT5, a T5-based hypernetwork that generates task-specific parameters for a frozen T5 model.
While hypertuning is not directly competitive with full fine-tuning or parameter-efficient fine-tuning, since it consists of only a single pass, we show that parameters generate from hypertuning can serve as better strong initializations for further parameter-efficient fine-tuning, with faster convergence and better final performance.

Training a hypernetwork is challenging for several reasons, one of them being the requirement for the model to output a large number of parameters, which often involves using a large neural network module or parameter-output head.
In Chapter 5, we addressed this issue by introducing an additional stage of training (\text{hypertraining}) to initialize these parameter-generation modules.
Ideally, we want to rely heavily on the pretrained language model when generating parameters, rather than introducing new parameters.
In Chapter 6, we conducted an investigation into using Gisting \cite{gisting} for hypertuning.
Gisting is an efficient method for adapating decoder Transformers to generate soft prefixes through only a modification of the causal attention mask and no newly introduced parameters, and initially appears to be a promising approach for using large language models as hypernetworks.
Our conclusions on this approach were mixed.
While we found that Gisting-based hypernetworks generally perform poorly compared to instruction-tuned models, or in some cases even few-shot prompted models, we demonstrate that hyperpretraining with Gisting and incorporating downstream model adaptation can lead to improved performance.
Additionally, compressing few-shot examples into Gists still leads to efficiency gains at inference time over few-shot prompting.
Overall, we found that Gisting may not be the most promising approach for LLM-based hypernetworks, despite its intial and intuitive appeal.

The last two years have seen a significant surge in interest in the workings and applications of large language models.
We have seen that model capabilities continue to scale across different dimensions (model size, training data, data quality via curation or collection), and we can expect these models to be placed in a wider array of applications over time.
As language models, and increasingly multi-modal models, start to be deployed in everyday applications, potentially in manners invisible to the end-user, both the academic and industry research communities desire better methods for imparting more capability and exerting finer-grain control over the behavior of such AI systems.
The field currently has a wide range of methods for incorporating knowledge from data into models: from direct model modifications such as fine-tuning, instruction tuning, and RLHF, to more indirect or inference-time methods such as few-shot prompting, prompt engineering and rejection sampling.
This remains a rich area of research, with new discoveries of interactions between these methods, and we should expect that there is still much for us to learn about transfer learning in large language models.
